People over trust AI-generated medical responses and view them to be as valid as doctors, despite low accuracy

This paper presents a comprehensive analysis of how AI-generated medical responses are perceived and evaluated by non-experts. A total of 300 participants gave evaluations for medical responses that were either written by a medical doctor on an online healthcare platform, or generated by a large language model and labeled by physicians as having high or low accuracy. Results showed that participants could not effectively distinguish between AI-generated and Doctors' responses and demonstrated a preference for AI-generated responses, rating High Accuracy AI-generated responses as significantly more valid, trustworthy, and complete/satisfactory. Low Accuracy AI-generated responses on average performed very similar to Doctors' responses, if not more. Participants not only found these low-accuracy AI-generated responses to be valid, trustworthy, and complete/satisfactory but also indicated a high tendency to follow the potentially harmful medical advice and incorrectly seek unnecessary medical attention as a result of the response provided. This problematic reaction was comparable if not more to the reaction they displayed towards doctors' responses. This increased trust placed on inaccurate or inappropriate AI-generated medical advice can lead to misdiagnosis and harmful consequences for individuals seeking help. Further, participants were more trusting of High Accuracy AI-generated responses when told they were given by a doctor and experts rated AI-generated responses significantly higher when the source of the response was unknown. Both experts and non-experts exhibited bias, finding AI-generated responses to be more thorough and accurate than Doctors' responses but still valuing the involvement of a Doctor in the delivery of their medical advice. Ensuring AI systems are implemented with medical professionals should be the future of using AI for the delivery of medical advice.

==> main <==
\begin{thebibliography}{10}

\bibitem{Edelman}
2023 edelman trust barometer special report: Trust and health.
\newblock 2023.

\bibitem{adams2023leveraging}
L.~C. Adams, D.~Truhn, F.~Busch, A.~Kader, S.~M. Niehues, M.~R. Makowski, and K.~K. Bressem.
\newblock Leveraging gpt-4 for post hoc transformation of free-text radiology reports into structured reporting: a multilingual feasibility study.
\newblock {\em Radiology}, page 230725, 2023.

\bibitem{ali2023potential}
H.~Ali.
\newblock The potential of gpt-4 as a personalized virtual assistant for bariatric surgery patients.
\newblock {\em Obesity Surgery}, pages 1--1, 2023.

\bibitem{ali2023performance}
R.~Ali, O.~Y. Tang, I.~D. Connolly, P.~L. Zadnik~Sullivan, J.~H. Shin, J.~S. Fridley, W.~F. Asaad, D.~Cielo, A.~A. Oyelese, C.~E. Doberstein, et~al.
\newblock Performance of chatgpt and gpt-4 on neurosurgery written board examinations.
\newblock {\em medRxiv}, pages 2023--03, 2023.

\bibitem{beam2023artificial}
A.~L. Beam, J.~M. Drazen, I.~S. Kohane, T.-Y. Leong, A.~K. Manrai, and E.~J. Rubin.
\newblock Artificial intelligence in medicine, 2023.

\bibitem{bender2021dangers}
E.~M. Bender, T.~Gebru, A.~McMillan-Major, and S.~Shmitchell.
\newblock On the dangers of stochastic parrots: Can language models be too big?
\newblock In {\em Proceedings of the 2021 ACM conference on fairness, accountability, and transparency}, pages 610--623, 2021.

\bibitem{brown2020language}
T.~Brown, B.~Mann, N.~Ryder, M.~Subbiah, J.~D. Kaplan, P.~Dhariwal, A.~Neelakantan, P.~Shyam, G.~Sastry, A.~Askell, et~al.
\newblock Language models are few-shot learners.
\newblock {\em Advances in neural information processing systems}, 33:1877--1901, 2020.

\bibitem{bubeck2023sparks}
S.~Bubeck, V.~Chandrasekaran, R.~Eldan, J.~Gehrke, E.~Horvitz, E.~Kamar, P.~Lee, Y.~T. Lee, Y.~Li, S.~Lundberg, et~al.
\newblock Sparks of artificial general intelligence: Early experiments with gpt-4.
\newblock {\em arXiv preprint arXiv:2303.12712}, 2023.

\bibitem{buccinca2021trust}
Z.~Bu{\c{c}}inca, M.~B. Malaya, and K.~Z. Gajos.
\newblock To trust or to think: cognitive forcing functions can reduce overreliance on ai in ai-assisted decision-making.
\newblock {\em Proceedings of the ACM on Human-Computer Interaction}, 5(CSCW1):1--21, 2021.

\bibitem{cadamuro2023potentials}
J.~Cadamuro, F.~Cabitza, Z.~Debeljak, S.~De~Bruyne, G.~Frans, S.~M. Perez, H.~Ozdemir, A.~Tolios, A.~Carobene, and A.~Padoan.
\newblock Potentials and pitfalls of chatgpt and natural-language artificial intelligence models for the understanding of laboratory medicine test results. an assessment by the european federation of clinical chemistry and laboratory medicine (eflm) working group on artificial intelligence (wg-ai).
\newblock {\em Clinical Chemistry and Laboratory Medicine (CCLM)}, (0), 2023.

\bibitem{chen2023utility}
S.~Chen, B.~H. Kann, M.~B. Foote, H.~J. Aerts, G.~K. Savova, R.~H. Mak, and D.~S. Bitterman.
\newblock The utility of chatgpt for cancer treatment information.
\newblock {\em medRxiv}, pages 2023--03, 2023.

\bibitem{cheng2023potential}
K.~Cheng, Z.~Sun, Y.~He, S.~Gu, and H.~Wu.
\newblock The potential impact of chatgpt/gpt-4 on surgery: will it topple the profession of surgeons?
\newblock {\em International Journal of Surgery}, pages 10--1097, 2023.

\bibitem{devlin2018bert}
J.~Devlin, M.-W. Chang, K.~Lee, and K.~Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language understanding.
\newblock {\em arXiv preprint arXiv:1810.04805}, 2018.

\bibitem{fitzpatrick2017delivering}
K.~K. Fitzpatrick, A.~Darcy, and M.~Vierhile.
\newblock Delivering cognitive behavior therapy to young adults with symptoms of depression and anxiety using a fully automated conversational agent (woebot): a randomized controlled trial.
\newblock {\em JMIR mental health}, 4(2):e7785, 2017.

\bibitem{he2023will}
Y.~He, H.~Tang, D.~Wang, S.~Gu, G.~Ni, and H.~Wu.
\newblock Will chatgpt/gpt-4 be a lighthouse to guide spinal surgeons?
\newblock {\em Annals of Biomedical Engineering}, pages 1--4, 2023.

\bibitem{hirosawa2023diagnostic}
T.~Hirosawa, Y.~Harada, M.~Yokose, T.~Sakamoto, R.~Kawamura, and T.~Shimizu.
\newblock Diagnostic accuracy of differential-diagnosis lists generated by generative pretrained transformer 3 chatbot for clinical vignettes with common chief complaints: A pilot study.
\newblock {\em International Journal of Environmental Research and Public Health}, 20(4):3378, 2023.

\bibitem{hisan2023chatgpt}
U.~K. Hisan and M.~M. Amri.
\newblock Chatgpt and medical education: A double-edged sword.
\newblock {\em Journal of Pedagogy and Education Science}, 2(01):71--89, 2023.

\bibitem{holmes2023evaluating}
J.~Holmes, Z.~Liu, L.~Zhang, Y.~Ding, T.~T. Sio, L.~A. McGee, J.~B. Ashman, X.~Li, T.~Liu, J.~Shen, et~al.
\newblock Evaluating large language models on a highly-specialized topic, radiation oncology physics.
\newblock {\em arXiv preprint arXiv:2304.01938}, 2023.

\bibitem{hosny2018artificial}
A.~Hosny, C.~Parmar, J.~Quackenbush, L.~H. Schwartz, and H.~J. Aerts.
\newblock Artificial intelligence in radiology.
\newblock {\em Nature Reviews Cancer}, 18(8):500--510, 2018.

\bibitem{hutto2014vader}
C.~Hutto and E.~Gilbert.
\newblock Vader: A parsimonious rule-based model for sentiment analysis of social media text.
\newblock In {\em Proceedings of the international AAAI conference on web and social media}, volume~8, pages 216--225, 2014.

\bibitem{jacobs2021designing}
M.~Jacobs, J.~He, M.~F.~Pradier, B.~Lam, A.~C. Ahn, T.~H. McCoy, R.~H. Perlis, F.~Doshi-Velez, and K.~Z. Gajos.
\newblock Designing ai for trust and collaboration in time-constrained medical decisions: A sociotechnical lens.
\newblock In {\em Proceedings of the 2021 chi conference on human factors in computing systems}, pages 1--14, 2021.

\bibitem{jakesch2023human}
M.~Jakesch, J.~T. Hancock, and M.~Naaman.
\newblock Human heuristics for ai-generated language are flawed.
\newblock {\em Proceedings of the National Academy of Sciences}, 120(11):e2208839120, 2023.

\bibitem{ayers2023jama}
M.~D. John W.~Ayers, Adam~Poliak.
\newblock Comparing physician and artificial intelligence chatbot responses to patient questions posted to a public social media forum.
\newblock {\em JAMA Internal Medicine}, 2023.

\bibitem{kahr2023seems}
P.~K. Kahr, G.~Rooks, M.~C. Willemsen, and C.~C. Snijders.
\newblock It seems smart, but it acts stupid: Development of trust in ai advice in a repeated legal decision-making task.
\newblock In {\em Proceedings of the 28th International Conference on Intelligent User Interfaces}, pages 528--539, 2023.

\bibitem{kung2023performance}
T.~H. Kung, M.~Cheatham, A.~Medenilla, C.~Sillos, L.~De~Leon, C.~Elepa{\~n}o, M.~Madriaga, R.~Aggabao, G.~Diaz-Candido, J.~Maningo, et~al.
\newblock Performance of chatgpt on usmle: Potential for ai-assisted medical education using large language models.
\newblock {\em PLoS digital health}, 2(2):e0000198, 2023.

\bibitem{Landi_2023}
H.~Landi.
\newblock Himss23: Epic taps microsoft to integrate generative ai into ehrs with stanford, uc san diego as early adopters, Apr 2023.

\bibitem{lee2023benefits}
P.~Lee, S.~Bubeck, and J.~Petro.
\newblock Benefits, limits, and risks of gpt-4 as an ai chatbot for medicine.
\newblock {\em New England Journal of Medicine}, 388(13):1233--1239, 2023.

\bibitem{levine2023diagnostic}
D.~M. Levine, R.~Tuwani, B.~Kompa, A.~Varma, S.~G. Finlayson, A.~Mehrotra, and A.~Beam.
\newblock The diagnostic and triage accuracy of the gpt-3 artificial intelligence model.
\newblock {\em medRxiv}, pages 2023--01, 2023.

\bibitem{liu2023deid}
Z.~Liu, X.~Yu, L.~Zhang, Z.~Wu, C.~Cao, H.~Dai, L.~Zhao, W.~Liu, D.~Shen, Q.~Li, et~al.
\newblock Deid-gpt: Zero-shot medical text de-identification by gpt-4.
\newblock {\em arXiv preprint arXiv:2303.11032}, 2023.

\bibitem{maliha21AIliab}
G.~Maliha, S.~Gerke, I.~G. Cohen, and R.~B. Parikh.
\newblock Artificial intelligence and liability in medicine.
\newblock {\em The Milbank Quarterly}, 99(3):629--647, 2021.

\bibitem{Mehnen2023.04.20.23288859}
L.~Mehnen, S.~Gruarin, M.~Vasileva, and B.~Knapp.
\newblock Chatgpt as a medical doctor? a diagnostic accuracy study on common and rare diseases.
\newblock {\em medRxiv}, 2023.

\bibitem{murphy2023generative}
C.~Murphy and F.~P. Thomas.
\newblock Generative ai in spinal cord injury research and care: Opportunities and challenges ahead.
\newblock {\em The Journal of Spinal Cord Medicine}, 46(3):341--342, 2023.

\bibitem{neely2021health}
S.~Neely, C.~Eldredge, and R.~Sanders.
\newblock Health information seeking behaviors on social media during the covid-19 pandemic among american social networking site users: survey study.
\newblock {\em Journal of medical Internet research}, 23(6):e29802, 2021.

\bibitem{nori2023capabilities}
H.~Nori, N.~King, S.~M. McKinney, D.~Carignan, and E.~Horvitz.
\newblock Capabilities of gpt-4 on medical challenge problems.
\newblock {\em arXiv preprint arXiv:2303.13375}, 2023.

\bibitem{oh2023chatgpt}
N.~Oh, G.-S. Choi, and W.~Y. Lee.
\newblock Chatgpt goes to operating room: Evaluating gpt-4 performance and its potential in surgical education and training in the era of large language models.
\newblock {\em medRxiv}, pages 2023--03, 2023.

\bibitem{openai2023gpt4}
OpenAI.
\newblock Gpt-4 technical report, 2023.

\bibitem{perlis2023application}
R.~H. Perlis.
\newblock Application of gpt-4 to select next-step antidepressant treatment in major depression.
\newblock {\em medRxiv}, pages 2023--04, 2023.

\bibitem{rao2023assessing}
A.~S. Rao, M.~Pang, J.~Kim, M.~Kamineni, W.~Lie, A.~K. Prasad, A.~Landman, K.~Dryer, and M.~D. Succi.
\newblock Assessing the utility of chatgpt throughout the entire clinical workflow.
\newblock {\em medRxiv}, pages 2023--02, 2023.

\bibitem{sallam2023chatgpt}
M.~Sallam.
\newblock Chatgpt utility in healthcare education, research, and practice: systematic review on the promising perspectives and valid concerns.
\newblock In {\em Healthcare}, volume~11, page 887. MDPI, 2023.

\bibitem{singhal2022large}
K.~Singhal, S.~Azizi, T.~Tu, S.~S. Mahdavi, J.~Wei, H.~W. Chung, N.~Scales, A.~Tanwani, H.~Cole-Lewis, S.~Pfohl, et~al.
\newblock Large language models encode clinical knowledge.
\newblock {\em arXiv preprint arXiv:2212.13138}, 2022.

\bibitem{szmuda2020readability}
T.~Szmuda, C.~{\"O}zdemir, S.~Ali, A.~Singh, M.~T. Syed, and P.~S{\l}oniewski.
\newblock Readability of online patient education material for the novel coronavirus disease (covid-19): a cross-sectional health literacy study.
\newblock {\em Public health}, 185:21--25, 2020.

\bibitem{tanaka2023performance}
Y.~Tanaka, T.~Nakata, K.~Aiga, T.~Etani, R.~Muramatsu, S.~Katagiri, H.~Kawai, F.~Higashino, M.~Enomoto, M.~Noda, et~al.
\newblock Performance of generative pretrained transformer on the national medical licensing examination in japan.
\newblock {\em medRxiv}, pages 2023--04, 2023.

\bibitem{alpaca}
R.~Taori, I.~Gulrajani, T.~Zhang, Y.~Dubois, X.~Li, C.~Guestrin, P.~Liang, and T.~B. Hashimoto.
\newblock Stanford alpaca: An instruction-following llama model.
\newblock \url{https://github.com/tatsu-lab/stanford_alpaca}, 2023.

\bibitem{teebagy2023improved}
S.~Teebagy, L.~Colwell, E.~Wood, A.~Yaghy, and M.~Faustina.
\newblock Improved performance of chatgpt-4 on the okap exam: A comparative study with chatgpt-3.5.
\newblock {\em medRxiv}, pages 2023--04, 2023.

\bibitem{thirunavukarasu2023large}
A.~J. Thirunavukarasu, D.~S.~J. Ting, K.~Elangovan, L.~Gutierrez, T.~F. Tan, and D.~S.~W. Ting.
\newblock Large language models in medicine.
\newblock {\em Nature medicine}, 29(8):1930--1940, 2023.

\bibitem{thoppilan2022lamda}
R.~Thoppilan, D.~De~Freitas, J.~Hall, N.~Shazeer, A.~Kulshreshtha, H.-T. Cheng, A.~Jin, T.~Bos, L.~Baker, Y.~Du, et~al.
\newblock Lamda: Language models for dialog applications.
\newblock {\em arXiv preprint arXiv:2201.08239}, 2022.

\bibitem{touvron2023llama}
H.~Touvron, T.~Lavril, G.~Izacard, X.~Martinet, M.-A. Lachaux, T.~Lacroix, B.~Rozi{\`e}re, N.~Goyal, E.~Hambro, F.~Azhar, et~al.
\newblock Llama: Open and efficient foundation language models.
\newblock {\em arXiv preprint arXiv:2302.13971}, 2023.

\bibitem{Turner_2023}
B.~E. Turner.
\newblock Epic, microsoft bring generative ai to ehrs, Apr 2023.

\bibitem{vamathevan2019applications}
J.~Vamathevan, D.~Clark, P.~Czodrowski, I.~Dunham, E.~Ferran, G.~Lee, B.~Li, A.~Madabhushi, P.~Shah, M.~Spitzer, et~al.
\newblock Applications of machine learning in drug discovery and development.
\newblock {\em Nature reviews Drug discovery}, 18(6):463--477, 2019.

\bibitem{van2023effect}
R.~van Kessel, I.~Kyriopoulos, B.~L.~H. Wong, and E.~Mossialos.
\newblock The effect of the covid-19 pandemic on digital health--seeking behavior: Big data interrupted time-series analysis of google trends.
\newblock {\em Journal of Medical Internet Research}, 25:e42401, 2023.

\bibitem{wrigley2021objective}
N.~Wrigley~Kelly, K.~Murray, C.~McCarthy, and D.~O’Shea.
\newblock An objective analysis of quality and readability of online information on covid-19.
\newblock {\em Health and Technology}, 11(5):1093--1099, 2021.

\bibitem{zhou2023evaluation}
Z.~Zhou.
\newblock Evaluation of chatgpt's capabilities in medical report generation.
\newblock {\em Cureus}, 15(4), 2023.

\bibitem{zimmerman2021health}
M.~S. Zimmerman.
\newblock Health information-seeking behavior in the time of covid-19: information horizons methodology to decipher source path during a global pandemic.
\newblock {\em Journal of Documentation}, 77(6):1248--1264, 2021.

\end{thebibliography}

